Mining Attribute-Based Access Control Policies from Logs

Attribute-based access control (ABAC) provides a high level of flexibility that promotes security and information sharing. ABAC policy mining algorithms have potential to significantly reduce the cost of migration to ABAC, by partially automating the development of an ABAC policy from information about the existing access-control policy and attribute data. This paper presents an algorithm for mining ABAC policies from operation logs and attribute data. To the best of our knowledge, it is the first algorithm for this problem.

==> generative.tex <==
\section{Algorithm Based on Generative Model}
\label{sec:algorithm:generative}

Another approach to this problem is to apply a machine learning algorithm
that uses a statistical approach, based upon a generative model, to find
the policy that is most likely to generate the behavior (usage of
permissions) observed in the logs.  This approach is inspired by Molloy
{\it et al.}'s work on mining RBAC policies and simple ABAC policies from
logs \cite{molloy12generative}, using Rosen-Zvi et al.'s algorithm for
learning author-topic models \cite{rosenzvi10learning}.

The author-topic model (ATM) is a probabilistic generative model for
collections of discrete data, such as documents \cite{rosenzvi10learning}.
ATM assumes the following process to generate a document $d$: for each word
$w$ in $d$, an author $a$ is randomly chosen, and then a topic $t$ is
chosen from a multinomial distribution over topics specific to the author
$a$, and then the word $w$ is chosen from a multinomial distribution over
words specific to the selected topic $t$.  The inputs to the ATM algorithm
are a set of authors, a set of documents, a function giving the set of
authors of each document, and the number of topics.  The ATM algorithm
finds a probability distribution relating authors to topics (i.e., how
likely each author is to write about each topic) and a probability
distribution relating topics to words (i.e., how likely each word is to be
used in text on each topic), such that the process described above, with
these probability distributions, is likely to generate the given documents.

Molloy {\it et al.}  use ATM to mine meaningful roles from logs and user
attribute data.  They employ the following correspondence
\cite{molloy12generative}: authors correspond to a restricted form of user
attribute expressions (specifically, user attribute expressions with at
most three conjuncts of the form ``{\it attribute}={\it value}''), topics
correspond to roles, words correspond to permissions, and documents
correspond to users (i.e., for each user $u$, there is a document
containing the permissions from the log entries for user $u$).  For the
document corresponding to user $u$, the set of authors is the set of user
attribute expressions (UAEs) satisfied by $u$.  With this correspondence,
the ATM finds a probability distribution $\phi_1$ relating UAEs to roles
(i.e., $\phi_1(e,r)$ is the probability that users satisfying UAE $e$ are
members of role $r$) and a probability distribution $\phi_2$ relating roles
to permissions (i.e., $\phi_2(r,p)$ is the probability that role $r$ has
permission $p$).  For each user $u$, the probability distributions
$\phi_1(e,r)$ for each UAE $e$ satisfied by $u$ are averaged.  Together,
the results form a probability distribution $\hat\phi_1$ relating users to
roles (i.e., $\hat\phi_1(u,r)$ is the probability that user $u$ is a member
of role $r$).  Finally, the probability distributions $\hat\phi_1$ and
$\phi_2$ are discretized to obtain a user-role assignment and a
role-permission assignment.

% Note that the resulting policy is an RBAC policy, not an ABAC policy, in
% the sense that the user-role assignment is defined by enumerating the users
% in each role, not by associating a UAE with each role.  Indeed, a UAE that
% exactly characterizes the set of members of a role might not even exist.

%Note that multiple UAEs may correspond to a high probability of membership
%in the same role, achieving the effect of disjunction, so disjunction
%within a UAE is unnecessary.

To adapt this approach to mine ABAC policies from logs and attribute data,
a new correspondence between the components of the author-topic model and
components of the access control model is needed, to accommodate the
following differences between our problem and theirs: the goal is to
generate an ABAC policy, not a meaningful RBAC policy; resource attribute
data, as well as user attribute data, is available; attributes can be
multi-valued, and set relations can be used in attribute expressions; and
constraints relating user attributes and resource attributes are allowed.

We propose the following correspondence.  The basic idea is to modify the
correspondence in \cite{molloy12generative} so that resources are treated
the same way as users, because in our framework, users and resources both
have attributes.  Another reason that users and resources need to be
treated together is the presence of constraints: users and resources must
be associated with rules in a coordinated way, not independently.  Thus,
resources are tupled with users, instead of being tupled with operations to
form permissions.  Authors correspond to tuples $\tuple{\uae, \rae, \con}$,
where $\uae$ is a user attribute expression with at most $b_u$ conjuncts,
$\rae$ is a resource attribute expression with at most $b_r$ conjuncts, and
$\con$ is a constraint with at most $b_c$ atomic constraints.  Furthermore,
(1) each conjunct in $\uae$ or $\rae$ may contain only one value,
specifically, one atomic value or one set of size at most $b_s$, depending
on whether the attribute is single-valued or multi-valued, and (2) each
user attribute and each resource attribute appear in at most one atomic
constraints in $\con$.  Disjunction (i.e., conjuncts with multiple values)
is introduced later, by ``merging'' sets of rules, as described below.
% our case studies contain at least one place where such merging is needed,
% namely, for the conjunct "type in {schedule budget}" in rule
% leaderScheduleBudget in project-management.abac.  the case studies do not
% contain any rules in which a set in a conjunct for a multi-valued attribute 
% is not a singleton set, so b_s=1 is sufficient.
In experiments, we take $b_u=2$, $b_r=2$, $b_c=2$, and $b_s=1$; these are
the smallest values sufficient to express our case study policies.  Topics
correspond to rules.  Words correspond to operations.  Documents correspond
to user-resource pairs; the document corresponding to a user-resource pair
$\tuple{u,r}$ is the sequence of operations performed (according to the
log) by user $u$ on resource $r$.  For the document corresponding to
$\tuple{u,r}$, the set of authors is the set of $\tuple{\uae, \rae, \con}$
tuples such that $u\models\uae \land r\models\rae \land u,r\models\con$.

%Note that $\tuple{\uae, \rae, \con}$ tuples that are not satisfied by any
%user-resource tuples will not appear in any author lists document and hence
%should not appear in the input to the algorithm. Nevertheless, the number
%of authors that appear in the input may be very large, perhaps
%prohibitively large for some problem instances.

The results of the ATM learning algorithm are a set of $k$ topics, and two
families of probability distributions $\theta$ and $\phi$.  For each author
$a$, $\theta_a$ is a probability distribution over topics, such that
$\theta_{a,t}$ is the probability that author $a$ will select to write
about topic $t$.  For each topic $t$, $\phi_t$ is a probability
distribution over words, such that $\phi_{t,w}$ is the probability that an
author writing on topic $t$ will use word $w$.  A discretization algorithm,
taken from Algorithm 1 in \cite{molloy12generative}, is used to obtain an
ABAC policy from the topics and probability distributions.  The details of
discretization algorithm, written in our notation, appear in Figure
\ref{fig:discretizationalg}. The inputs are: the input $I$ to the policy
mining problem defined in Section \ref{sec:problem}, the families of
probability distributions $\theta$ and $\phi$ described above, the maximum
number of iterations $\maxIter$, the author set $A$, the word set $W$, the
number of topics $k$.  The integer array $AT$ used in the algorithm defines
the discretized author-topic assignment; specifically, author $a$ is
associated with the $AT[a]$ topics that have the largest probability
according to $\theta_a$.  Similarly, the array $TW$ defines the discretized
topic-word assignment; specifically, topic $t$ is is associated with the
$TW[t]$ words that have the largest probability according to $\phi_t$.  A
set of rules is constructed from $AT$ and $TW$ by the $\constructABACRules$
function defined in Figure \ref{fig:constructabac}.  For each topic $t$,
and for each author $\tuple{\uae,\rae,\con}$ that is associated with $t$ by
$AT$, the rule $\tuple{\uae,\rae,O,\con}$ is included in the rule set,
where $O$ is the set of words that are associated with $t$ by $TW$.

To reduce the policy's WSC and improve its quality, $\constructABACRules$
invokes a variant of the $\mergerules$ function defined in Figure
\ref{fig:mergerules}.  This variant, called $\mergerulesgen$, is obtained
from $\mergerules$ by replacing the validity test $\mean{\rhomerge}
\subseteq \up_0$
% the analogue of the validity test would be \mean{\rhomerge}\subseteq\up(L).
(which is inappropriate here because over-assignments are allowed) with a
test that merging does not change the meaning of the policy, namely,
$\mean{\rhomerge} \subseteq \mean{\Rho}$.
% note that $\mean{\Rho}$ is invariant (i.e., it does not change during
% execution of mergerules), so we can compute \mean{\Rho} on entry to the
% function and cache the result.
% is there any reason not to merge rules whenever possible to reduce WSC?
% e.g., should rules with different usage frequencies not be merged?

% the following describes a computationally cheaper version of merging.
% however, I guess it might miss some opportunities for merging.

% To reduce the policy size, if a set of rules can be represented more
% compactly by a single rule that uses disjunction (i.e., conjuncts with
% multiple values), then we replace that set of rules with that single
% rule. A set of rules can be merged if their constraints and operations are
% the same, and their $\uae$'s and $\rae$'s conjuncts are almost the same,
% except there exists one user or resource attribute, such that the
% corresponding conjuncts of the set of rules on this attribute are
% different.  Pseudocode for merging rules appears in Figure
% \ref{fig:abac-from-logs:mergerules}.

The discretization algorithm aims to find values for $AT$ and $TW$ that
maximize a policy quality metric.  We use the policy quality metric defined
in equation \ref{eq:Qpolicy} in Section
\ref{sec:problem}.  The algorithm is based on
% considering that it uses a random number generator, I don't know
% why they call it ``deterministic''.
annealing. The algorithm begins with a random initialization of $AT$ and
$TW$, and iteratively updates them until the updates converge or the
maximum number of iteration is reached. In each iteration, the algorithm
first tries to update each $AT[a]$ with a new value that differs from the
current value by at most $\epsilon$, where $\epsilon$ is a parameter of the
annealing process.  If the updated value results in an ABAC policy with a
higher quality, then the new value is accepted (by storing it in
$\ATtmp[a]$ and later assigning it to $AT[a]$). Otherwise, the new value is
accepted with a probability drawn from the probability distribution
Pr[exp((Q($\pi, L$) - Q($\pi', L$)))/$T$)/$Z$], where $Z$ is a
normalization factor, and $T$ is the temperature.  The initial temperature
$T_0$ is relatively high, and the temperature is decreased with rate
$\gamma$ in each iteration, where $T_0$ and $\gamma$ are parameters to the
annealing process.  $TW$ is updated similarly.  All accepted updates are
applied to $AT$ and $TW$ simultaneously at the end of each iteration, by
the assignment $AT = \ATtmp$ and a similar assignment for $TW$.  This
algorithm is greedy in the sense that it considers only associations in
which some number of the highest-ranked topics or words are associated with
an author or topic, respectively; consequently, it might be unable to
produce an optimal discretization in some cases.

% The policy metric $Q(\pi, L)$ used in our discretization algorithm is based
% on WSC, as in Section \ref{sec:abac-from-acl:problem}, except with
% additional terms to penalize under-assignments and over-assignments, with
% weights specified by parameters $w_u$ and $w_o$, respectively:
% \begin{equation}
%   Q(\pi, L) = \wsc(\pi) \times (1
%   \begin{array}[t]{@{}l@{}}
%     + \frac{w_u|\underassign(\pi,L)|_L}{|\up(L)|}
%     + \frac{w_o|\overassign(\pi,L)|}{|\up(L)|}
%   )
%   \end{array}
%   \label{eq:abac-from-logs:Qpol}
% \end{equation}
% where
% \begin{eqnarray}
%   \underassign(\pi,L) &=& \up(L)\setminus\mean{\pi}\label{eq:underassign2}\\
%   \overassign(\pi,L) &=& \mean{\pi}\setminus\up(L)\label{eq:overassign2}
% \end{eqnarray}
% As in Section \ref{sec:abac-from-acl:problem}, smaller values indicate
% higher quality.  Note that the numbers of under-assignments and
% over-assignments are measured relative to $|\up(L)|$, and that this
% definition uses the frequency-weighted size of $\underassign(\pi,L)$,
% making the policy quality metric sensitive to usage frequency.  The
% distance metric for RBAC policies in \cite{molloy12generative} is similar
% but slightly simpler, because it does not take policy size into account.
% The analogue for ABAC is obtained by omitting the factor of $\wsc(\pi)$ and
% omitting ``1 +''.

% I reduced the indentation levels from ~~~~ to ~~~ to eliminate some
% overfull lines.
\begin{figure} [htbp]
\resetlnum
\begin{tabbing}
~~~~\= \function\ Discretization($I, \theta, \phi, \maxIter, A, W, k$)\\
%\> Input:\\
%\>$L$: operation log\\
%\> $\theta$: probability distributions of authors ($\tuple{\uae, \rae, \con}$ tuples) to topics(rules)\\
%\>$\phi$: probability distributions of topics over words(operations)\\
%\>$\gamma$: temperature decreasing rate\\
%\>maxIter: the maximum number of iterations\\
%\>Output:\\
%\> $\pi_{res}$: the result ABAC policy\\
\lnum\> $AT$ = new Vector(), $TW$ = new Vector()\\
\lnum\> \forloop\ $a$ = 1 to $|A|$\\
\lnum\>~~~\= $AT[a] = \randomint(0, k)$\\
\lnum\> \eforloop\ \\
\lnum\> \forloop\ $t$ = 1 to $k$\\
\lnum\>~~~\= $TW[t] = \randomint(0, |W|)$\\
\lnum\> \eforloop\ \\
\lnum\> $\Rho = \constructABACRules(\theta, \phi, AT, TW, A)$\\
\lnum\> $\pi = I[8 \rightarrow \Rho]$\\
\lnum\> $T$ = $T_0$\\
\lnum\> $i = 0$\\
\lnum\> \whileloop\ $i \leq \maxIter$\\
\lnum\>~~~\= $\ATtmp = AT.\Copy()$\\
\lnum\>\> \forloop\ $a$ = 1 to $|A|$\\
\lnum\>\>~~~\= $AT' = AT.\Copy()$\\
%\lnum\>\>\> $t'_a\leftarrow$[max(0,$t_a$ - $\epsilon$), min($k$, $t_a$ + $\epsilon$)]\\
\lnum\>\>\> $AT'[a] = \randomint(max(0, AT[a] - \epsilon), min(k, AT[a] + \epsilon))$\\
\lnum\>\>\> $\Rho' = \constructABACRules(\theta, \phi, AT', TW, A)$\\
\lnum\>\>\> $\pi' = I[8 \rightarrow \Rho']$\\
\lnum\>\>\> \ifstmt\ $Q(\pi',  \pi_{in}.L) < Q(\pi,  \pi_{in}.L)$ \\
\lnum\>\>\>~~~\= $\ATtmp[a] = AT'[a]$\\
\lnum\>\>\> \elsestmt\ \\
\lnum\>\>\>\> \ifstmt\ $\random(0, 1) \leq {\rm Pr}[{\rm exp}((Q(\pi', L) - Q(\pi, L)))/T)/Z]$\\
\lnum\>\>\>\>~~~\= $\ATtmp[a] = AT'[a]$\\
\lnum\>\>\>\> \eifstmt\ \\
\lnum\>\>\> \eifstmt\ \\
\lnum\>\> \eforloop\ \\
\lnum\>\> /* Perform a similar updating process for $TW$ */ \\
\lnum\>\> $\Rho = \constructABACRules(\theta, \phi, \ATtmp, \TWtmp, A)$\\
\lnum\>\> $\pi = I[8 \rightarrow \Rho]$\\
\lnum\>\> \ifstmt\ $AT = \ATtmp$ \andstmt\ $TW = \TWtmp$\\
\lnum\>\>\> \breakstmt\ \\
\lnum\>\> \eifstmt\ \\
\lnum\>\> $AT = \ATtmp$; $TW = \TWtmp$\\
\lnum\>\> $T = \gamma T$\\
\lnum\>\> $i = i + 1$\\
\lnum\> \ewhileloop\ \\
\lnum\> \return\ $\pi$
\end{tabbing}
\caption{Discretization algorithm.  $\random(x,y)$ returns a random number
  in the range $[x,y)$. $\randomint(i,j)$ returns a random integer in the
  range $[i,j]$.  $t[i \rightarrow v]$ denotes the tuple obtained from
  tuple $t$ by changing the value of the $i$'th component to $v$. }
\label{fig:discretizationalg}
\end{figure}

\begin{figure}[htbp]
\resetlnum
\begin{tabbing}
~~~~\=\function\ $\constructABACRules(\theta, \phi, AT, TW, A)$\\
\lnum\> $\Rho$ = new Set()\\
\lnum\> \forloop\ $a$ in $A$ \\
\lnum\>~~~~\= $T$ = \= the set containing the topics corresponding to\\
\lnum\>\>\>            the $AT[a]$ largest values of $\theta_a$ \\
\lnum\>\> \forloop\ $t$ in $T$\\
\lnum\>\>~~~~\= $O$ = \= the set containing the words corresponding to\\
\lnum\>\>\>\>            the $TW[t]$ largest values of $\phi_t$\\
\lnum\>\>\> $\tuple{\uae, \rae, \con} = a$\\
\lnum\>\>\> $\rho = \tuple{\uae, \rae, O, \con}$\\
\lnum\>\>\> $\Rho.\add(\rho)$\\
\lnum\>\> \eforloop\ \\
\lnum\> \eforloop\ \\
\lnum\> $\mergerulesgen(\Rho)$\\
\lnum\> \return\ $\Rho$
\end{tabbing}
\caption{Construct an ABAC policy based on an author-topic assignment and a
  topic-word assignment.  }
\label{fig:constructabac}
\end{figure}


%\begin{figure}[htbp]
%\resetlnum
%\begin{tabbing}
%~~~~\=\function\ $\constructABACPolicy(\theta, \phi, AT, TW, A, \pi)$\\
%\lnum\> $\Rho$ = new Set()\\
%\lnum\> \forloop\ $a$ in $A$ \\
%\lnum\>~~~~\= $T$ = the set containing the topics corresponding to the $AT[a]$ largest values of $\theta_a$ \\
%\lnum\>\> \forloop\ $t$ in $T$\\
%\lnum\>\>~~~~\= $O$ = the set containing the words corresponding to the $TW[t]$ largest values of $\phi_t$\\
%\lnum\>\>\> $\tuple{\uae, \rae, \con} = a$\\
%\lnum\>\>\> $\rho = \tuple{\uae, \rae, O, \con}$\\
%\lnum\>\>\> $\Rho.\add(\rho)$\\
%\lnum\>\> \eforloop\ \\
%\lnum\> \eforloop\ \\
%\lnum\> $\mergerulesgen(\Rho)$\\
%\lnum\> \return\ $\tuple{\pi.U, \pi.R, \pi.\Op, \pi.\Au, \pi.\Ar, \pi.\uad, \pi.\rad,\Rho}$
%\end{tabbing}
%\caption{Construct an ABAC policy based on an author-topic assignment and a
%  topic-word assignment.  }
%\label{fig:abac-from-logs:constructabac}
%\end{figure}

% \begin{figure}[htbp]
% \resetlnum
% \begin{tabbing}
% ~~~~\= \function\ $\mergerulesgen(\Rho)$\\
% \lnum\> $\Rho'$ = $\emptyset$\\
% \lnum\> \whileloop\ $\Rho \neq \Rho'$\\
% \lnum\>~~~~\=  \forloop\ $\rho$  \forloopin\ $\Rho$\\
% \lnum\>\>~~~~\= \removed\ = \false\\
% \lnum\>\>\> \forloop\ $\rho'$  \forloopin\ $\Rho\setminus\{\rho\}$\\
% \lnum\>\>\>~~~~\= \ifstmt\ $\con(\rho)=\con(\rho')\land \ops(\rho)=\ops(\rho')$\\
% \lnum\>\>\>\>~~~~\= \merged\ = \false \\
% \lnum\>\>\>\>\> \ifstmt\ $\rae(\rho) = \rae(\rho') \land \exists a_u \in \Au. \uae(\rho)(a_u)\neq \uae(\rho')(a_u)$\\
% \>\>\>\>\>~~~~\= ${} \land \forall a_u' \in \Au\setminus\{a_u\}. \uae(\rho)(a_u')= \uae(\rho')(a_u')$\\
% \lnum\>\>\>\>\>\>      $\rhomerge = \langle\uae(\rho)\union\uae(\rho'),\rae(\rho),\ops(\rho),\con(\rho)\rangle$\\
% \lnum\>\>\>\>\>\> \merged\ = true\\
% \lnum\>\>\>\>~~~~\= \elsestmt\ \ifstmt\ $\uae(\rho) = \uae(\rho') \land \exists a_r \in \Ar. (\rae(\rho)(a_r)\neq \rae(\rho')(a_r)$\\
% \>\>\>\>\>~~~~\= ${}\land \forall a_r' \in \Ar\setminus\{a_r\}. \rae(\rho)(a_r')= \rae(\rho')(a_r')$\\
% \lnum\>\>\>\>\>\>      $\rhomerge = \langle\uae(\rho),\rae(\rho)\union\rae(\rho'),\ops(\rho),\con(\rho)\rangle$\\
% \lnum\>\>\>\>\>\> \merged\ = \true\\
% \lnum\>\>\>\>\>\eifstmt\ \\
% \lnum\>\>\>\>\>\ifstmt\ \merged\ = \true \\
% \lnum\>\>\>\>\>\> $\Rho'$ = $\Rho'\union \{\rhomerge\}$\\
% \lnum\>\>\>\>\>\> $\Rho = \Rho\setminus\{\rho, \rho'\}$\\
% \lnum\>\>\>\>\>\> \removed\ = \true\\
% \lnum\>\>\>\>\>\> \breakstmt\ \\
% \lnum\>\>\>\>\>\eifstmt\ \\
% \lnum\>\>\>\>\eifstmt\ \\
% \lnum\>\>\> \eforloop\ \\
% \lnum\>\>\> \ifstmt\ \removed\ = \true\\
% \lnum\>\>\>\> \continuestmt\  \\
% \lnum\>\>\> \elsestmt\ \\
% \lnum\>\>\>\>$\Rho'$ = $\Rho'\union \{\rho\}$\\
% \lnum\>\>\>\eifstmt\ \\
% \lnum\>\> \eforloop\ \\
% \lnum\> \ewhileloop\ \\
% \lnum \return\ $\Rho'$\\
% \end{tabbing}
% \caption{Merge rules}
% \label{fig:abac-from-logs:mergerules}
% \end{figure}

Recall that the ATM algorithm takes the number $k$ of topics (i.e., the
desired number of rules in the policy) as an input.  In general, $k$ is not
known in advance.  A simple approach to determine a reasonable value of $k$
is to start with a low estimate and iteratively increase it, re-running the
entire algorithm each time, until the improvement in policy quality falls
below a threshold.  Developing an incremental version of the ATM algorithm
would be difficult, so the policy mining algorithm would executed from
scratch each time, making this approach inefficient.  It might be possible
to develop a more efficient search strategy for finding the smallest value
of $k$ that, when incremented, produces a below-threshold improvement in
policy quality.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% TeX-PDF-mode: t
%%% End: 

